Learning Intra-Batch Connections for Deep Metric Learning

The goal of metric learning is to learn a function that maps samples to a lower-dimensional space where similar samples lie closer than dissimilar ones. Particularly, deep metric learning utilizes neural networks to learn such a mapping. Most approaches rely on losses that only take the relations between pairs or triplets of samples into account, which either belong to the same class or two different classes. However, these methods do not explore the embedding space in its entirety. To this end, we propose an approach based on message passing networks that takes all the relations in a mini-batch into account. We refine embedding vectors by exchanging messages among all samples in a given batch allowing the training process to be aware of its overall structure. Since not all samples are equally important to predict a decision boundary, we use an attention mechanism during message passing to allow samples to weigh the importance of each neighbor accordingly. We achieve state-of-the-art results on clustering and image retrieval on the CUB-200-2011, Cars196, Stanford Online Products, and In-Shop Clothes datasets. To facilitate further research, we make available the code and the models at https://github.com/dvl-tum/intra_batch_connections.

==> tables/additional_parameters.tex <==
\begin{table*}[hbt!]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{@{}l|c|c|c|c}
\hline
 & \textbf{CUB-200-2011} &  \textbf{Cars196} & \textbf{Stanford Online Products} &  \textbf{In-shop Clothes}\\
\hline
Embedding layer bb CNN & 2,048,576 & 2,048,576 & 2,048,576 & 2,048,576 \\
FC-layer bb CNN & 51,200 & 50,274 & 5,806,134 & 2,050,0561\\
MPN Training & 3,458,288 & 6,619,548 & 9,211,904 & 5,463,552 \\
MPN Test & 3,417,088 & 3,417,088 & 3,417,088 & 3,417,088\\

\hline
\end{tabular}}
\caption{Performance of our approach using different embedding sizes on CUB-200-2011, Cars196, Stanford Online Products and In-Shop Clothes datasets. bb stands for backbone.}
\label{tab:add_params}
\end{table*}

==> tables/backbones.tex <==
\begin{table}[hbt!]
\centering
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{@{}l|cc|cc@{}}
\hline
& \multicolumn{2}{c}{CUB-200-2011} & \multicolumn{2}{c}{Cars196} \\
\hline
 & \textbf{R@1} &  \textbf{NMI} & \textbf{R@1} &  \textbf{NMI}\\
\hline
ResNet50 & 70.3 & 74.0 & \textbf{88.1} & \textbf{74.8} \\
DenseNet161 & \textbf{71.0} & \textbf{75.5} & \textbf{88.1} & 70.9 \\
\hline
\end{tabular}}
\caption{Performance of our approach using DenseNet201 as backbone architecture on CUB-200-2011 and Cars196 compared to ResNet50.}
\label{tab:backbone}
\end{table}


\iffalse
\begin{table}[hbt!]
\tiny
\centering
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{@{}l|cc|cc@{}}
\hline
& \multicolumn{2}{c}{CUB-200-2011} & \multicolumn{2}{c}{CARS196} \\ 
\hline
 & \textbf{R@1} &  \textbf{NMI} & \textbf{R@1} &  \textbf{NMI}\\
\hline
ResNet18 & 57.4 & 62.7 & 80.8 & 61.6 \\
ResNet34 & 62.5 & 65.2 & 84.2 & 67.9 \\
ResNet101 & 68.2 & 71.9 & 87.5 & 72.7 \\
ResNet152 & 68.6 & 72.6 & 85.8 & 71.5 \\
\hline
DenseNet161 & 72.5 & 75.5 & 86.7 & 71.9 \\
DenseNet169 & 68.8 & 71.9 & 87.2 & 70.4 \\
DenseNet201 & 71.0 & 75.5 & 88.1 & 70.9 \\
\hline
\end{tabular}}
\caption{Performance of our approach with different backbone architectures on CUB-200-2011, Cars196, Stanford Online Products and In-Shop Clothes datasets.}
\label{tab:backbone_old}
\end{table}
\fi

==> tables/different_num_classes_num_samples.tex <==
\begin{table}[hbt!]
\centering
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{@{}l|cccccc@{}}
\hline
 & 2 / 27 & 3 / 18 & 6 / 9 &  9 / 6 & 18 / 3 & Sampler\\
\hline
CUB-200-2011 & 67.2 & 68.4 &  68.1 & 66.1 & 65.3 & 70.3 \\
\hline
\hline
 & 3 / 12 & 4 / 9 & 6 / 6 &  9 / 4 & 12 / 3 & Sampler\\
\hline
Cars196 & 83.7 & 85.9 & 86.5 & 86.9 & 86.7 & 87.7 \\
\hline
\end{tabular}}
\caption{R@1  on CUB-200-2011 and Cars196 datasets with respect to different number of classes and samples (number of classes / number of samples), when the batch size is kept approximately the same.}
\label{tab:diff_num_classes_samples}
\end{table}

==> tables/larger_batches.tex <==
\begin{table}[hbt!]
\centering
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{@{}l|cc|cc@{}}
%& \multicolumn{2}{c}{CUB-200-2011} & \multicolumn{2}{c}{Cars196} & \multicolumn{2}{c}{Stanford Online Products} & \multicolumn{2}{c}{In-Shop Clothes} \\ 
\hline
 & \multicolumn{2}{c}{CUB-200-2011} & \multicolumn{2}{c}{Cars196} \\
\hline
 & \textbf{R@1} &  \textbf{NMI} & \textbf{R@1} &  \textbf{NMI} \\ % \textbf{R@1} &  \textbf{NMI}& \textbf{R@1} &  \textbf{NMI}\\
\hline
Ours$^{512*}$ & 70.3 & 73.2 & 87.9 & 74.1 \\
ProxyAnchor$^{512*}$ \cite{DBLP:conf/cvpr/KimKCK20} & 67.0 & - & 84.6 & - \\
Ours$^{512\dagger}$ & 68.7 & 72.6 & 88.6 & 72.2 \\
ProxyAnchor$^{512\dagger}$ \cite{DBLP:conf/cvpr/KimKCK20} & 68.8 & - & 86.1 & - \\
\hline
\end{tabular}}
\caption{Performance of our approach using larger batches. \dagger indicates batches in the range of the batch size of Proxy Anchor \cite{DBLP:conf/cvpr/KimKCK20}, * indicates batch sizes in the range of our batch sizes.}
\label{tab:larger_batches}
\end{table}

==> tables/resnet50_comp.tex <==
\begin{table*}[hbt!]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{@{}l|ccccc|ccccc@{}}
\hline
& \multicolumn{5}{c}{CUB-200-2011} & \multicolumn{5}{c}{Cars196} \\
\hline
 & \textbf{R@1} &  \textbf{R@2} & \textbf{R@4} &  \textbf{R@8} & \textbf{NMI} & \textbf{R@1} &  \textbf{R@2} & \textbf{R@4} &  \textbf{R@8}& \textbf{NMI}\\
\hline
Proxy Anchor$^{512}$ \cite{DBLP:conf/cvpr/KimKCK20} & 69.7 & 80.0 & 87.0 & 92.4 & - & 87.7 & 92.9 & 95.8 & 97.9 & -\\
%Ours^{512} & 70.3 & 73.2 & 87.9 & 74.1 & 81.1 & 92.6 & 93.8\\
Ours$^{512}$ &  \textbf{70.3} & \textbf{80.3} & \textbf{87.6} & \textbf{92.7}  & \textbf{74.0} & \textbf{88.1} & \textbf{93.3} & \textbf{96.2} & \textbf{98.2} & \textbf{74.8} \\
\hline
\end{tabular}}
\caption{Performance of Proxy Anchor \cite{DBLP:conf/cvpr/KimKCK20} using a ResNet50 backbone compared to our performance.}
\label{tab:resnet50}
\end{table*}

==> tables/training_tricks.tex <==
\begin{table}[hbt!]
\centering
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{@{}l|cc|cc|cc@{}}

\hline
\textbf{} & \multicolumn{2}{c}{CUB-200-2011} & \multicolumn{2}{c}{CARS196} \\ \hline
\textbf{Training Tricks} &  \textbf{R@1} & \textbf{NMI} &  \textbf{R@1} & \textbf{NMI} \\
\hline
Baseline & 54.4 & 63.1 & 70.9 & 64.0\\
+ temperature & 65.8 & 70.8 & 82.2 & 70.6 \\
+ max pooling & 66.2 & 70.6 & 84.4 & 66.5  \\
+ sampler & 68.7 & 72.7 & 87.3 & 70.7 \\
+ Random erasing & 69.3 & 72.9 & 87.6 & 70.9 \\
- auxiliary loss (CE) & 68.1 & 72.0 & 88.4 & 69.0\\
\hline
Solely CE, no training tricks & 52.2 & 62.4 \\
Solely CE, all training tricks & 67.5 & 69.8 \\
\hline
 \end{tabular}}
\caption{Training Tricks of training.}
\label{tab:training_tricks}
\end{table}
